Restoring Images in Adverse Weather Conditions via Histogram Transformer

Transformer-based image restoration methods in adverse weather have achieved significant progress. Most of them use self-attention along the channel dimension or within spatially fixed-range blocks to reduce computational load. However, such a compromise results in limitations in capturing long-range spatial features. Inspired by the observation that the weather-induced degradation factors mainly cause similar occlusion and brightness, in this work, we propose an efficient Histogram Transformer (Histoformer) for restoring images affected by adverse weather. It is powered by a mechanism dubbed histogram self-attention, which sorts and segments spatial features into intensity-based bins. Self-attention is then applied across bins or within each bin to selectively focus on spatial features of dynamic range and process similar degraded pixels of the long range together. To boost histogram self-attention, we present a dynamic-range convolution enabling conventional convolution to conduct operation over similar pixels rather than neighbor pixels. We also observe that the common pixel-wise losses neglect linear association and correlation between output and ground-truth. Thus, we propose to leverage the Pearson correlation coefficient as a loss function to enforce the recovered pixels following the identical order as ground-truth. Extensive experiments demonstrate the efficacy and superiority of our proposed method. We have released the codes in Github.

==> fig_tex/boxplot.tex <==

\begin{figure*}[t]
  \centering
   \includegraphics[width=1\linewidth]{fig/boxplot.pdf}
  % \vspace{-6mm}
   \caption{The boxplot of the mean opinion score for each method. }
   \label{fig:boxplot}
   % \vspace{-3mm}
\end{figure*}


==> fig_tex/complex/complex.tex <==

\begin{figure}[t]
  \centering    
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0 0 0,clip, width=1\linewidth]{fig/other_tasks/complex/0058_lq.png}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch0_lq.png}
    \end{subfigure}
    
    \vspace{-0mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch1_lq.png}
    \end{subfigure}
    \end{minipage}
    \vspace{-2mm}
    \subcaption[]{Input}
    \label{fig:stats-a}
    \end{minipage}
    %
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_weatherdiff.png}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch0_weatherdiff.png}
    \end{subfigure}
    
    \vspace{-0mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch1_weatherdiff.png}
    \end{subfigure}
    \end{minipage}
    \vspace{-2mm}
    \subcaption[]{WeatherDiff$_{128}$}
    \label{fig:stats-a}
    \end{minipage}
    %
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_ours__.jpeg}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch0_ours__.jpeg}
    \end{subfigure}
    
    \vspace{-0mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/complex/0058_patch1_ours__.jpeg}
    \end{subfigure}
    \end{minipage}
    \vspace{-2mm}
    \subcaption[]{Ours}
    \label{fig:stats-a}
    \end{minipage}
   % \includegraphics[width=1\linewidth]{fig/intro Diagram.pdf}
   \vspace{-4.5mm}
    \caption{Robustness against both snow and raindrop.}
   \vspace{-7mm}
   \label{fig:complex}
\end{figure}


==> fig_tex/other_tasks/other_tasks.tex <==

\begin{figure}[t]
  \centering    
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[trim=200 0 30 0,clip, width=1\linewidth]{fig/other_tasks/deblur/deblur_result_gt.jpg}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/deblur/deblur_result_patch0_gt.jpg}
    \end{subfigure}
    
    \vspace{-1mm}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/deblur/deblur_result_patch0_Restormer.jpg}
    \end{subfigure}
    
    \vspace{-1mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/deblur/deblur_result_patch0_ours.jpg}
    \end{subfigure}
    \end{minipage}
    \subcaption[]{GoPro}
    \label{fig:deblurring}
    \end{minipage}
    %
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/llie/llie_result_gt.png}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/llie/llie_result_patch0_gt.png}
    \end{subfigure}
    
    \vspace{-1mm}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/llie/llie_result_patch0_snr.png}
    \end{subfigure}
    
    \vspace{-1mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/llie/llie_result_patch0_ours.jpg}
    \end{subfigure}
    \end{minipage}
    \subcaption[]{LOLv1}
    \label{fig:enhancement}
    \end{minipage}
    %
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0 0 27,clip, width=1\linewidth]{fig/other_tasks/dehaze/dehaze_result_gt.png}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/dehaze/dehaze_result_patch0_gt.png}
    \end{subfigure}
    
    \vspace{-1mm}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/dehaze/dehaze_result_patch0_Dehamer.png}
    \end{subfigure}
    
    \vspace{-1mm}
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/other_tasks/dehaze/dehaze_result_patch0_ours.png}
    \end{subfigure}
    \end{minipage}
    \subcaption[]{SOTS-Outdoor}
    \label{fig:dehazing}
    \end{minipage}
   % \includegraphics[width=1\linewidth]{fig/intro Diagram.pdf}
   \vspace{-4mm}
    \caption{\textbf{Top to Down}: Ground-truth, baseline and ours.}
   \vspace{-3mm}
   \label{fig:other_tasks}
\end{figure}


==> fig_tex/raindrop/raindrop_1.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result//restormer/21_rain.png}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/transweather/21_rain.png}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/restormer/21_rain.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/wgws/21_rain.png}
    \caption{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/weatherdiff/21_rain.png}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}

  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/histoformer/21_rain.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/gt/21_rain.png}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/raindrop/raindrop_3.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result//restormer/27_rain.png}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/transweather/27_rain.png}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/restormer/27_rain.png}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/wgws/27_rain.png}
    \caption{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/weatherdiff/27_rain.png}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}

  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/histoformer/27_rain.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/gt/27_rain.png}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/raindrop/supple_raindrop-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{RaindropAttn~\cite{quan2019deep}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_patch0_15_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_patch1_15_rain.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of real-world raindrop removal on RainDrop~\cite{qian2018attentive}.}
  \label{fig:raindrop-supple-1}
\end{figure*}

==> fig_tex/raindrop/supple_raindrop-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/input_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/raindropattn_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{RaindropAttn~\cite{quan2019deep}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/restormer_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/transweather_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/chen_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/wgws_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/weatherdiff_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/histoformer_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_patch0_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_patch1_34_rain.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.325\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/raindrop/rect/gt_patch2_34_rain.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of real-world raindrop removal on RainDrop~\cite{qian2018attentive}.}
  \label{fig:raindrop-supple-2}
\end{figure*}

==> fig_tex/rainfog/supple_rainfog-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{MPRNet~\cite{Zamir2021mprnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_im_0343_s95_a05.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_patch0_im_0343_s95_a05.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_patch1_im_0343_s95_a05.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_patch0_im_0343_s95_a05.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_patch1_im_0343_s95_a05.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of rain streak and haze removal on Outdoor-Rain~\cite{li2019heavy}.}
  \label{fig:rainfog-supple-1}
\end{figure*}

==> fig_tex/rainfog/supple_rainfog-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{MPRNet~\cite{Zamir2021mprnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_im_0331_s80_a06.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_patch0_im_0331_s80_a06.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_patch1_im_0331_s80_a06.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_patch0_im_0331_s80_a06.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_patch1_im_0331_s80_a06.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of rain streak and haze removal on Outdoor-Rain~\cite{li2019heavy}.}
  \label{fig:rainfog-supple-2}
\end{figure*}

==> fig_tex/rainfog/supple_rainfog-3.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/input_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/mprnet_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{MPRnet~\cite{Zamir2021mprnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/restormer_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/transweather_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/chen_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/wgws_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_im_0326_s85_a06.jpg}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/weatherdiff_patch0_im_0326_s85_a06.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/histoformer_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_im_0326_s85_a06.png}
  \end{subfigure}
  \hspace{-1mm}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/rainfog/rect/gt_patch0_im_0326_s85_a06.png}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparison of rain streak and haze removal on Outdoor-Rain~\cite{li2019heavy}.}
  \label{fig:rainfog-supple-3}
\end{figure*}

==> fig_tex/realrain/supple_realrain-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/input_122.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/mprnet_122.png}
  \end{subfigure}
    \subcaption[]{MPRNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/restormer_122.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/transweather_122.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/chen_122.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/wgws_122.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/weatherdiff_122.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/histoformer_122.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of real-world rain streak and haze removal from Internet-Data~\cite{wang2019spatial}.}
  \label{fig:realrain-supple-1}
\end{figure*}

==> fig_tex/realrain/supple_realrain-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/input_137.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/mprnet_137.png}
  \end{subfigure}
    \subcaption[]{MPRNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/restormer_137.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/transweather_137.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/chen_137.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/wgws_137.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/weatherdiff_137.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realrain/histoformer_137.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of real-world rain streak and haze removal from Internet-Data~\cite{wang2019spatial}.}
  \label{fig:realrain-supple-2}
\end{figure*}

==> fig_tex/realsnow/realsnow_1.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00113.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00113.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00113.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00113.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00113.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00113.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00113.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_10.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_07513.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_07513.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_07513.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_07513.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_07513.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_07513.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_07513.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_11.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/snow_animal_00072.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/snow_animal_00072.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/snow_animal_00072.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/snow_animal_00072.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/snow_animal_00072.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/snow_animal_00072.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/snow_animal_00072.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_12.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.29\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/snow_animal_00093.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/snow_animal_00093.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/snow_animal_00093.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/snow_animal_00093.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/snow_animal_00093.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/snow_animal_00093.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.29\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/snow_animal_00093.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_13.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/snow_animal_02555.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/snow_animal_02555.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/snow_animal_02555.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/snow_animal_02555.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/snow_animal_02555.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/snow_animal_02555.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/snow_animal_02555.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_14.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/snow_crossing_00015.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/snow_crossing_00015.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/snow_crossing_00015.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/snow_crossing_00015.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/snow_crossing_00015.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/snow_crossing_00015.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/snow_crossing_00015.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_15.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter_weather_02459.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter_weather_02459.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter_weather_02459.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter_weather_02459.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter_weather_02459.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter_weather_02459.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter_weather_02459.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_16.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter__street_01703.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter__street_01703.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter__street_01703.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter__street_01703.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter__street_01703.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter__street_01703.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter__street_01703.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_17.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter__street_01695.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter__street_01695.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter__street_01695.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter__street_01695.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter__street_01695.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter__street_01695.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter__street_01695.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_18.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter__street_04364.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter__street_04364.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter__street_04364.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter__street_04364.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter__street_04364.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter__street_04364.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter__street_04364.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_19.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter__street_06380.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter__street_06380.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter__street_06380.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter__street_06380.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter__street_06380.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter__street_06380.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter__street_06380.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_2.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00416.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00416.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00416.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00416.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00416.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00416.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00416.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_20.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter_weather_05884.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter_weather_05884.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter_weather_05884.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter_weather_05884.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter_weather_05884.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter_weather_05884.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter_weather_05884.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_3.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00426.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00426.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00426.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00426.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00426.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00426.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00426.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_4.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00675.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00675.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00675.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00675.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00675.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00675.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00675.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_5.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00864.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00864.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00864.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00864.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00864.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00864.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00864.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_6.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_04954.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_04954.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_04954.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_04954.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_04954.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_04954.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_04954.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_7.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_05318.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_05318.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_05318.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_05318.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_05318.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_05318.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_05318.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_8.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_06860.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_06860.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_06860.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_06860.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_06860.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_06860.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_06860.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/realsnow_9.tex <==
\begin{figure*}
  \centering
  % \begin{subfigure}{0.495\linewidth}
  %   \includegraphics[width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_07197.jpg}
  %   \caption{Input}
  %   \label{fig:short-a}
  % \end{subfigure}
  
  % \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_07197.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_07197.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_07197.jpg}
    \caption{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_07197.jpg}
    \caption{WGWSNet~\cite{zhu2023learning_wgwsnet}}
    \label{fig:short-d}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_07197.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.495\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_07197.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-1.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/winter_weather_05884.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter_weather_05884.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter_weather_05884.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
    \vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-1}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-2.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/first_snow_00416.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00416.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00416.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-2}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-3.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/first_snow_00426.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00426.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00426.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-3}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-4.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/first_snow_00675.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00675.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00675.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-4}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-5.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/first_snow_00864.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/first_snow_00864.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.375\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/first_snow_00864.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-5}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-6.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/snow_animal_00093.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/snow_animal_00093.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.245\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/snow_animal_00093.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-6}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-7.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/input/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/ddmsnet/winter__street_06380.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/restormer/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/transweather/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/chen/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/wgws/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/weatherdiff/winter__street_06380.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/realsnow/histoformer/winter__street_06380.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-7}
\end{figure*}

==> fig_tex/realsnow/supple_realsnow-8.tex <==
\begin{figure*}
\vspace{-5mm}
  \centering
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/input/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/ddmsnet/sidewalk winter -grayscale -gray_07197.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/restormer/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/transweather/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/chen/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/wgws/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/weatherdiff/sidewalk winter -grayscale -gray_07197.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1mm}
  \begin{minipage}{0.455\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 20mm 0 0,clip,width=1\linewidth]{fig/result/realsnow/histoformer/sidewalk winter -grayscale -gray_07197.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
\vspace{-3mm}
  \caption{A visual comparison of real-world desnowing on Snow100K~\cite{liu2018desnownet}.}
  \label{fig:realsnow-supple-8}
\end{figure*}

==> fig_tex/snow/snow_2.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_05086.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_05086.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_05086.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_05086.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_05086.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_05086.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/snow_3.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_05419.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_05419.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_05419.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_05419.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_05419.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_05419.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/snow_4.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_05754.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_05754.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_05754.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_05754.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_05754.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_05754.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/snow_5.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_06010.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_06010.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_06010.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_06010.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_06010.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_06010.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/snow_6.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_06036.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_06036.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_06036.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_06036.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_06036.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_06036.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/snow_7.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/input/winter_weather_06207.jpg}
    \caption{Input}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/transweather/winter_weather_06207.jpg}
    \caption{TransWeather~\cite{valanarasu2022transweather}}
    \label{fig:short-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/restormer/winter_weather_06207.jpg}
    \caption{Restormer~\cite{zamir2022restormer}}
    \label{fig:short-c}
  \end{subfigure}
  
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/weatherdiff/winter_weather_06207.jpg}
    \caption{WeatherDiff~\cite{ozdenizci2023restoring}}
    \label{fig:short-d}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/histoformer/winter_weather_06207.png}
    \caption{Ours}
    \label{fig:short-e}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.33\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/gt/winter_weather_06207.jpg}
    \caption{Ground-truth}
    \label{fig:short-f}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

==> fig_tex/snow/supple_snow-1.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_winter_weather_05086.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_patch0_winter_weather_05086.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_patch1_winter_weather_05086.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_winter_weather_05086.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_patch0_winter_weather_05086.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_patch1_winter_weather_05086.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_patch0_winter_weather_05086.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_patch1_winter_weather_05086.jpg}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparisons of desnowing on Snow100K-L~\cite{liu2018desnownet}.}
  \label{fig:snow-supple-1}
\end{figure*}

==> fig_tex/snow/supple_snow-2.tex <==
\begin{figure*}
  \centering
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/input_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{Input}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_winter_weather_06010.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_patch0_winter_weather_06010.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/ddmsnet_patch1_winter_weather_06010.png}
  \end{subfigure}
    \subcaption[]{DDMSNet~\cite{zhang2021deep}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/restormer_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{Restormer~\cite{zamir2022restormer}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/transweather_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{TransWeather~\cite{valanarasu2022transweather}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/chen_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/wgws_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{WGWS-Net~\cite{zhu2023learning_wgwsnet}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/weatherdiff_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{WeatherDiff$_{64}$~\cite{ozdenizci2023restoring}}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_winter_weather_06010.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_patch0_winter_weather_06010.png}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/histoformer_patch1_winter_weather_06010.png}
  \end{subfigure}
    \subcaption[]{Ours}
    \end{minipage}
  \hspace{-1.5mm}
  \begin{minipage}{0.330\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_patch0_winter_weather_06010.jpg}
  \end{subfigure}
  \hspace{-1.5mm}
  \begin{subfigure}{0.493\linewidth}
    \includegraphics[width=1\linewidth]{fig/result/snow/rect/gt_patch1_winter_weather_06010.jpg}
  \end{subfigure}
    \subcaption[]{Ground-truth}
    \end{minipage}
  \caption{A visual comparisons of desnowing on Snow100K-L~\cite{liu2018desnownet}.}
  \label{fig:snow-supple-2}
\end{figure*}

==> fig_tex/stats/stat.tex <==

\begin{figure}[t]
  \centering
  \begin{minipage}{0.242\linewidth}
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/snow/beautiful_smile_01949.jpg}
    \end{subfigure}
     \begin{subfigure}{0.51\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/snow/hist_beautiful_smile_01949.pdf}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/snow/snow_global.pdf}
    \end{subfigure}
    \subcaption[]{Snow100K-L}
    \label{fig:stats-a}
    \end{minipage}
    %
  \begin{minipage}{0.242\linewidth}
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[trim=350 0 0 0,clip, width=1\linewidth]{fig/stats/rain_streaks/212.png}
    \end{subfigure}
     \begin{subfigure}{0.51\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/rain_streaks/hist_212.pdf}
    \end{subfigure}
    
    \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/rain_streaks/rain_streaks_global.pdf}
    \end{subfigure}
    \subcaption[]{RainDS~[3]}
    \label{fig:stats-b}
    \end{minipage}
    %
  \begin{minipage}{0.242\linewidth}
    \centering
    \begin{subfigure}{0.45\linewidth}
    \includegraphics[trim=100 0 0 0,clip, width=1\linewidth]{fig/stats/raindrop/54_rain.png}
    \end{subfigure}
    \hfill
     \begin{subfigure}{0.51\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/raindrop/hist_54_rain.pdf}
    \end{subfigure}
    
    \begin{subfigure}{\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/raindrop/raindrop_global.pdf}
    \end{subfigure}
    \subcaption[]{RainDrop}
    \label{fig:stats-b}
    \end{minipage}
    %
  \begin{minipage}{0.242\linewidth}
  \vspace{-1mm}
  \begin{minipage}{0.4\linewidth}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[trim=0 200 0 0,clip, width=1\linewidth]{fig/stats/fog/lindau_000004_000019_leftImg8bit_foggy_beta_0.01.png}
    \end{subfigure}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[trim=0 200 0 0,clip, width=1\linewidth]{fig/stats/fog/lindau_000004_000019_leftImg8bit_transmittance_beta_0.01.png}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.51\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/fog/hist_lindau_000004_000019_leftImg8bit_foggy_beta_0.01.pdf}
    \end{subfigure}
    \end{minipage}
    
     \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/fog/fog_global.pdf}
    \end{subfigure}
    \vspace{-5mm}
    \subcaption[]{\tiny Foggy Cityscapes}
    \label{fig:fog_stats}
    \end{minipage}
   % \includegraphics[width=1\linewidth]{fig/intro Diagram.pdf}
   \vspace{-4mm}
    \caption{\textbf{1st row}: A randomly sampled image and the histogram on it.
    \textbf{2rd row}: Histogram of all samples.}
   \vspace{-3mm}
   \label{fig:stats}
\end{figure}


==> fig_tex/stats/stat_fog.tex <==

\begin{figure}[t]
  \centering    
  \begin{minipage}{0.325\linewidth}
  \begin{minipage}{0.54\linewidth}
    \begin{subfigure}{1\linewidth}
    \includegraphics[trim=0 0 0 0,clip, width=1\linewidth]{fig/stats/fog/hist_lindau_000004_000019_leftImg8bit_foggy_beta_0.01.pdf}
    \end{subfigure}
    \end{minipage}
    \hspace{-1mm}
  \begin{minipage}{0.44\linewidth}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/fog/lindau_000004_000019_leftImg8bit_foggy_beta_0.01.png}
    \end{subfigure}
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/fog/lindau_000004_000019_leftImg8bit_transmittance_beta_0.01.png}
    \end{subfigure}
    \end{minipage}
    \hfill
     \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1\linewidth]{fig/stats/fog/fog_global.pdf}
    \end{subfigure}
    \subcaption[]{\tiny Foggy Cityscapes-DBF}
    \label{fig:stats-a}
    \end{minipage}
   % \includegraphics[width=1\linewidth]{fig/intro Diagram.pdf}
   \vspace{-4mm}
    \caption{Histogram for different depths.}
   \vspace{-5mm}
   \label{fig:fog_stats}
\end{figure}


==> tab_sec/complexity.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
\footnotesize
\renewcommand\arraystretch{1.4}
\tabcolsep=1.mm
  \centering
  \caption{The performances of deweathering, space and computational complexities of the existing deweathering methods. The PSNR and SSIM are tested on Outdoor-Rain~\cite{li2019heavy} and the results of FLOPs are computed on the inputs of 256$\times$256.}
  % \vspace{-3mm}
    \begin{tabular}{lrrrrrrrr}
    \toprule
          & Restormer~\cite{zamir2022restormer} & All-in-One~\cite{li2020all} & TransWeather~\cite{valanarasu2022transweather} & Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval} & WGWS-Net~\cite{zhu2023learning_wgwsnet} & WeatherDiff$_{64}$~\cite{ozdenizci2023restoring} & WeatherDiff$_{128}$~\cite{ozdenizci2023restoring} & Histoformer \\
    \midrule
    PNSR  & 30.03 & 24.71 & 28.83 & 28.47 & 28.65 & 29.64 & 29.72 & 32.08 \\
    SSIM  & 0.9215 & 0.8980 & 0.9000 & 0.9107 & 0.9207 & 0.9312 & 0.9216 & 0.9389 \\
    \#Parameter & 26.10M & 44.00M & 38.05M & 28.71M & 5.19M & 82.92M & 85.56M & 16.73M \\
    FLOPs & 140.99G & 12.26G & 12.24G & 49.22G & 13.61G & 475.16G & 263.45G & 88.55G \\
    \bottomrule
    \end{tabular}%
  \label{tab:complexity}%
  % \vspace{-4mm}
\end{table}%


==> tab_sec/complexity2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[tbp]
\tiny
\renewcommand\arraystretch{1.4}
\tabcolsep=0.1mm
  \centering
  \caption{The performances of deweathering, space and computational complexities of the existing deweathering methods. The PSNR and SSIM are tested on Outdoor-Rain~\cite{li2019heavy} and the results of FLOPs are computed on the inputs of 256$\times$256.}
  % \vspace{-3mm}
    \begin{tabular}{lrrrrrrr}
    \toprule
          & All-in-One~\cite{li2020all} & TransWeather~\cite{valanarasu2022transweather} & Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval} & WGWS-Net~\cite{zhu2023learning_wgwsnet} & WeatherDiff$_{64}$~\cite{ozdenizci2023restoring} & WeatherDiff$_{128}$~\cite{ozdenizci2023restoring} & Ours \\
    \midrule
    PNSR  & 24.71 & 28.83 & 28.47 & 28.65 & 29.64 & 29.72 & 32.08 \\
    SSIM  & 0.8980 & 0.9000 & 0.9107 & 0.9207 & 0.9312 & 0.9216 & 0.9389 \\
    \#Param & 44.00M & 38.05M & 28.71M & 5.19M & 82.92M & 85.56M & 16.61M \\
    FLOPs & 12.26G & 12.24G & 49.22G & 13.61G & 475.16G & 263.45G & 91.59G \\
    \bottomrule
    \end{tabular}%
  \label{tab:complexity}%
  % \vspace{-4mm}
\end{table}%


==> tab_sec/niqe.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\tiny
\renewcommand\arraystretch{1.4}
\tabcolsep=0.mm
  \centering
  \caption{The metrics comparison of real-world adverse weather removal for non-reference image quality assessment on Snow100K~\cite{liu2018desnownet}.}
  % \vspace{-3mm}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
          & Input & DDMSNet~\cite{zhang2021deep} & Restormer~\cite{zamir2022restormer} & TransWeather~\cite{valanarasu2022transweather} & Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval} & WGWS-Net~\cite{zhu2023learning_wgwsnet} & WeatherDiff$_{64}$~\cite{ozdenizci2023restoring} & WeatherDiff$_{128}$~\cite{ozdenizci2023restoring} & Histoformer \\
    \midrule
    NIQE$\downarrow$ & 2.68  & 2.62  & 2.67  & 3.58  & 3.47  & 3.51  & 3.30  & 3.32  & \textbf{1.80} \\
    BRISQUE$\downarrow$ & 18.37 & 16.34 & 18.14 & 19.64 & 20.98 & 21.23 & 20.67 & 20.73 & \textbf{13.53} \\
    \bottomrule
    \end{tabular}%
  \label{tab:niqe}%
  % \vspace{-4mm}
\end{table}%


==> tab_sec/niqe2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\tiny
\renewcommand\arraystretch{1.4}
\tabcolsep=0.4mm
  \centering
  \caption{The metrics comparison of real-world adverse weather removal for non-reference image quality assessment on Snow100K~\cite{liu2018desnownet}.}
  % \vspace{-3mm}
    \begin{tabular}{lrrrrrrrr}
    \toprule
          & Input &  TransWeather~\cite{valanarasu2022transweather} & Chen \textit{et al}.~\cite{Chen2022MultiWeatherRemoval} & WGWS-Net~\cite{zhu2023learning_wgwsnet} & WeatherDiff$_{64}$~\cite{ozdenizci2023restoring} & WeatherDiff$_{128}$~\cite{ozdenizci2023restoring} & Ours \\
    \midrule
    NIQE$\downarrow$ & 2.68  & 3.58  & 3.47  & 3.51  & 3.30  & 3.32  & \textbf{1.80} \\
    BRISQUE$\downarrow$ & 18.37 & 19.64 & 20.98 & 21.23 & 20.67 & 20.73 & \textbf{13.53} \\
    \bottomrule
    \end{tabular}%
  \label{tab:niqe}%
  % \vspace{-4mm}
\end{table}%


==> tab_sec/tab_conf.tex <==
% Table generated by Excel2LaTeX from sheet 'rebuttal_eccv'
\begin{table}[t]
\vspace{-3mm}
\renewcommand\arraystretch{0.4}
\tabcolsep=0.4mm
\scriptsize
  \centering
  \caption{Detection confidences [\%] in Fig.~7 and of 2 baselines. }
    Abbreviation notations. P is Person. D is Door. C is Coat. J is Jeans. B is Building. \\
    \begin{tabular}{llllllllllllll}
    \toprule
    Label & P     & P     & D     & D     & C     & J     & D     & B     & B     & B     & B     & B     & B \\
    \midrule
    Degraded & 87    & 74    & 75    & 74    & 61    & 69    & 0     & 89    & 81    & 79    & 72    & 72    & 0 \\
    W/ ours\(_{\textcolor{c6}{\tiny \Delta}}\) & 84\(_{\textcolor{c6}{\tiny\textbf{-3}}}\)    & 80\(_{\textcolor{c6}{\tiny\textbf{+6}}}\)    & 77\(_{\textcolor{c6}{\tiny\textbf{+2}}}\)    & 77\(_{\textcolor{c6}{\tiny\textbf{+3}}}\)    & 68\(_{\textcolor{c6}{\tiny\textbf{+7}}}\)    & 71\(_{\textcolor{c6}{\tiny\textbf{+2}}}\)    & 59\(_{\textcolor{c6}{\tiny\textbf{+59}}}\)    & 86\(_{\textcolor{c6}{\tiny\textbf{-3}}}\)    & 83\(_{\textcolor{c6}{\tiny\textbf{+2}}}\)    & 81\(_{\textcolor{c6}{\tiny\textbf{+2}}}\)    & 77\(_{\textcolor{c6}{\tiny\textbf{+5}}}\)    & 77\(_{\textcolor{c6}{\tiny\textbf{+5}}}\)    & 55\(_{\textcolor{c6}{\tiny\textbf{+55}}}\) \\
    \midrule
    Restormer & 82    & 79    & 74    & 74    & 63    & 60    & 0     & 86    & 80    & 77    & 73    & 71    & 0 \\
    WeatherDiff & 82    & 80    & 72    & 76    & 66    & 70    & 55    & 84    & 80    & 77    & 77    & 69    & 0 \\
    \bottomrule
    \end{tabular}%
  \label{tab:fluctuating_conf}%
  \vspace{-6mm}
\end{table}%

==> tab_sec/tab_other_tasks.tex <==

% Table generated by Excel2LaTeX from sheet 'rebuttal_eccv'
\begin{table}[t]
\renewcommand\arraystretch{0.5}
\tabcolsep=0.4mm
\scriptsize
  \centering
  \caption{The PSNR/SSIM results of our methods on other tasks.}
  \vspace{-3mm}
\begin{subtable}[t]{0.32\linewidth}
        \caption{Deblur: GoPro}\label{tab:deblurring}%
        \vspace{-1mm}
    \begin{tabular}{cc}
    \toprule
    Restormer & Ours \\
    32.92 / 0.961 & 33.55 / 0.966 \\
    \bottomrule
    \end{tabular}%
    \end{subtable}
    \hfill
\begin{subtable}[t]{0.32\linewidth}
        \caption{Enhance: LOLv1}\label{tab:enhancement}%
        \vspace{-1mm}
    \begin{tabular}{cc}
    \toprule
    SNR & Ours \\
    24.61 / 0.842 & 24.96 / 0.849 \\
    \bottomrule
    \end{tabular}%
    \end{subtable}
    \hfill
\begin{subtable}[t]{0.32\linewidth}
        \caption{Dehaze: SOTS-Out.}\label{tab:dehazing}%
        \vspace{-1mm}
    \begin{tabular}{cc}
    \toprule
    Dehamer & Ours \\
    35.18 / 0.986 & 36.97 / 0.9891 \\
    \bottomrule
    \end{tabular}%
    \end{subtable}
  \label{tab:extra-data}%
  \vspace{-6mm}
\end{table}%



==> tab_sec/tab_runtime.tex <==
% Table generated by Excel2LaTeX from sheet 'rebuttal_eccv'
\begin{table}[t]
\renewcommand\arraystretch{0.4}
\tabcolsep=1.4mm
\scriptsize
  \centering
  \caption{Comparisons of runtime and model size on Nvidia V100.}
    \begin{tabular}{lrrrr}
    \toprule
          & Restormer & WeatherDiff$_{64}$ & WeatherDiff$_{128}$ & Ours \\
    \midrule
    PNSR~[dB]  & 30.03 & 29.64 & 29.72 & 32.08 \\
    \#Parameter~[M] & 26.10 & 82.92 & 85.56 & 16.73 \\
    Average runtime~[s] & 0.214 & 158.45 & 298.12 & 0.133 \\
    \bottomrule
    \end{tabular}%
  \label{tab:runtime}%
  \vspace{-3mm}
\end{table}%
